Robust Bipedal Locomotion: Leveraging Saltation Matrices for Gait Optimization

The ability to generate robust walking gaits on bipedal robots is key to their successful realization on hardware. To this end, this work extends the method of Hybrid Zero Dynamics (HZD) -- which traditionally only accounts for locomotive stability via periodicity constraints under perfect impact events -- through the inclusion of the saltation matrix with a view toward synthesizing robust walking gaits. By jointly minimizing the norm of the extended saltation matrix and the torque of the robot directly in the gait generation process, we demonstrate that the synthesized gaits are more robust than gaits generated with either term alone; these results are shown in simulation and on hardware for the AMBER-3M planar biped and the Atalante lower-body exoskeleton (both with and without a human subject). The end result is experimental validation that combining saltation matrices with HZD methods produces more robust bipedal walking in practice.

==> Sections/HZD_Old.tex <==

The hybrid zero dynamics (HZD) method of gait generation is a mathematical framework capable of synthesizing provably stable walking trajectories (gaits) via trajectory optimization \cite{grizzle20103d}. One of the main benefits of this method is that it directly accounts for discrete impact events by modeling the system as a hybrid system, constructed as a sequential series of continuous dynamics (which comprise the swing phase of walking) and discrete impact events (which describe the discrete dynamics that occurs during instantaneous impact events). The inclusion of feedback control transforms the passive hybrid system into a hybrid control system, defined as the tuple:
\begin{align}
    \mathcal{H}{C} = (\Gamma, \mathcal{D}, \mathcal{U}, \mathcal{S}, \Delta, FG),
\end{align}
where $\Gamma = \{V,E\}$ is a directed cycle with $V$ denoting the set of vertices describing continuous dynamics for unique sets of holonomic constraints, and $E$ denoting the set of edges, $e = (v_s \to v_t) \in E$, for each $v_s, v_t \in V$. The set of admissible domains is denoted by $\mathcal{D} = \{\mathcal{D}_v\}_{v \in V}$, which can be interpreted as the set of states realizable on the physical robot. The set of guards is denoted $\mathcal{S} = \{S_e \subset \mathcal{D}_{v_s} \}_{e \in E}$, and can be interpreted as the transition point from one domain to the next. The set of reset maps is denoted $\Delta = \{\Delta_e\}_{e \in E}$, with each reset map, $\Delta_e: \mathcal{S}_e \subset \mathcal{D}_{v_s} \to \mathcal{D}_{v_t}$, providing the post-impact state: $x^+ = \Delta_e(x^-)$. Lastly, $FG = (f_v, g_v)_{v \in V}$ denotes the set of control systems of the form $\dot{x} = f_v(x) + g_v(x)u$.

For ease of notation, the duration of this paper will assume that there is only one domain (describing the continuous swing phase) and a single discrete event (describing the instantaneous change in state caused by the swing foot impact). Thus, the system dynamics are described by:
\begin{align}
\mathcal{H}\mathcal{C} = 
    \begin{cases}
        \dot{x} = f(x) + g(x)u, & x \not \in \mathcal{S}, \\
        x^+ = \Delta x^-, & x \in \mathcal{S}.
    \end{cases}
\end{align}
For robotic systems with coordinates $q \in \mathcal{Q} \subset \R^n$, we take $x = (q, \dot{q})^{\top} \in T\mathcal{Q}$. The continuous-time dynamics of robotic systems is captured as:
\begin{align}
    D(q)\ddot{q} + H(q,\dot{q})\dot{q} = Bu.
\end{align}


For legged robotic systems with ground impacts, it is standard to derive the discrete impact map $\Delta$ assuming a rigid impact model \cite{grizzle20103d}. Specifically, a commonly used impact model introduces a contact impulse $\delta F$ into the dynamic model \cite{hurmuzlu1994rigid}:
\begin{align}
    D(q)\ddot{q} + H(q,\dot{q})\dot{q} = Bu + J(q)^{\top}\delta F.
\end{align}
Then, by integrating the dynamic equation over the instantaneous duration of the impact, we obtain:
\begin{align}
    D(q_e)(\dot{q}^+ - \dot{q}^-) = J(q_e)^{\top}F,
\end{align}
with $F := \int_{t^-}^{t^+} \delta F(\tau) d\tau$. Note that we use $q_e$ to represent the positions at impact, assuming that the position does not change during impact, i.e. $q_e := q^+ = R q^-$, with $R \in \R^{n \times n}$ being the relabeling matrix. In most cases, $R = I$. Additionally, it is assumed that the foot impacts the ground with a position of ``zero'' (on a flat foot). This is represented using the kinematic constraint:
\begin{align}
    J(q_e)\dot{q}^+ = 0.
\end{align}
These equations can be combined as:
\begin{align}
    \begin{bmatrix}
        D(q_e) & -J(q_e)' \\ J(q_e) & 0
    \end{bmatrix}
    \begin{bmatrix}
        \dot{q}^+ \\ F
    \end{bmatrix} = 
    \begin{bmatrix}
        D(q_e)\dot{q}^{-} \\ 0
    \end{bmatrix}
\end{align}
Note that by rearranging this system of equations, the reset mapping can be explicitly written as:
\begin{align}
    \Delta(x^-) := 
    \begin{bmatrix}
        Rq^- \\ (-D^{-1}J'(J D^{-1}J')^{-1} J + I)\dot{q}^-    
    \end{bmatrix}
\end{align}

\blue{
The \textbf{reset} map, $\Delta: \mathcal{S} \to \mathcal{D}$, maps states on the guard (termed pre-impact states) through a discrete transition to corresponding states in the continuous-time domain (termed the post-impact states). This reset map is often denoted,
\begin{align}
    x^+ = \Delta(x^-).
\end{align}
For robotic systems, the state can be decoupled into position and velocity terms, $x := [q, \dot{q}]^T \in \R^{2n}$ with $q, \dot{q} \in \R^n$. }

For bipedal systems, the guard (assuming a known and constant ground height of zero) is defined as:
\begin{align}
    \mathcal{S} := \{(q,\dot{q}): p_{\text{nsf}}^z(q) = 0, \dot{p}_{\text{nsf}}^z(q,\dot{q}) < 0\}
\end{align}
where $p_{\text{nsf}}^z: \mathcal{Q} \to \R$ denotes the vertical height of the non-stance foot and $\dot{p}_{\text{nsf}}^z(q,\dot{q}): \mathcal{Q} \times T\mathcal{Q} \to \R$ denotes the vertical component of the non-stance foot velocity.
